To Update or Not To Update?: Bandwidth-Efficient Intelligent Replacement Policies for DRAM Caches

This paper investigates intelligent replacement policies for improving the hit-rate of gigascale DRAM caches. Cache replacement policies are commonly used to improve the hit-rate of on-chip caches. The most effective replacement policies often require the cache to track per-line reuse state to inform their decision. A fundamental challenge on DRAM caches, however, is that stateful policies would require significant bandwidth to maintain per-line DRAM cache state. As such, DRAM cache replacement policies have primarily been stateless policies, such as always-install or probabilistic bypass. Unfortunately, we find that stateless policies are often too coarse-grain and become ineffective at the size and associativity of DRAM caches. Ideally, we want a replacement policy that can obtain the hit-rate benefits of stateful replacement policies, but keep the bandwidth-efficiency of stateless policies. In our study, we find that tracking per-line reuse state can enable an effective replacement policy that can mitigate common thrashing patterns seen in gigascale caches. We propose a stateful replacement/bypass policy called RRIP Age-On-Bypass (RRIP-AOB), that tracks reuse state for high-reuse lines, protects such lines by bypassing other lines, and Ages the state On cache Bypass. Unfortunately, such a stateful technique requires significant bandwidth to update state. To this end, we propose Efficient Tracking of Reuse (ETR). ETR makes state tracking efficient by accurately tracking the state of only one line from a region, and using the state of that line to guide the replacement decisions for other lines in that region. ETR reduces the bandwidth for tracking replacement state by 70%, and makes stateful policies practical for DRAM caches. Our evaluations with a 2GB DRAM cache, show that our RRIP-AOB and ETR techniques provide 18% speedup while needing less than 1KB of SRAM.

==> old6Adesign_wb.tex <==



%\section{Design: Dynamic Write Policy}
\section{Optimizing for Write Traffic}

\ignore{

We observe performance degradation for some write-heavy workloads (e.g., \textit{bc twi}). We find that this is primarily due to two reasons. First, our configuration assumes a write-sensitive non-volatile memory. Any increase in write traffic can delay the servicing of reads and cause longer read latency. And second, our default RRIP implementation sometimes causes increased write traffic compared to Always-Install, which can degrade performance significantly (-15\% for \textit{bc twi}). We investigate RRIP write policy in more detail.
}

%sometimes causes increased write traffic compared to Always-Install.




We find the major difference between Always-Install and RRIP is how the policies handle write-misses. With Always-Install, on a write-miss, lines are always installed, as in Figure~\ref{fig:writeback}(a). Such a Write-Allocate policy enables the cache to serve as a write buffer and reduce the number of writes to non-volatile memory. However, write-allocate on a direct-mapped cache will often evict lines that have reuse, so it can perform poorly. Meanwhile, RRIP on a write-miss treats write-miss and read-misses identically, and often bypasses write-misses. Bypassing for write-misses becomes a Write-No-Allocate policy, shown in Figure~\ref{fig:writeback}(b). Such a write-no-allocate policy optimizes for cache space, but, it can come at the cost of increased write traffic if writes have reuse. 



\begin{figure}[htb] 
%	\vspace{-0.15in}
    \vspace{.1in}
	\centering
	\includegraphics[width=1\columnwidth]{FIGURES/writeback.pdf}
%	\vspace{-0.10in}
	\caption{Write-Allocate vs. Write-No-Allocate. Write-Allocate can reduce writes to main memory, whereas Write-No-Allocate can prevent no-reuse writes from flooding the cache.}
	\label{fig:writeback} 
%	\vspace{-0.15in}
\end{figure}



\begin{figure*}[htb] 
	\vspace{-0.15in}
	\centering
	\includegraphics[height=1.5in]{GRAPHS/perf_wb.pdf}
	%\includegraphics[width=\columnwidth]{GRAPHS/bypass_perf.pdf}
	\vspace{-0.13in}
	
	\caption{Performance of ETR (Write Unaware), ETR (Allocate on Write-Miss), ETR (Dynamic Allocate on Write Miss) and State-in-SRAM (with Dynamic Allocate on Write Miss). ETR with Dynamic Allocate improves speedup to 19.4\%. }
	\label{fig:shipwb_perf} 
	\vspace{-0.15in}
\end{figure*}


Ideally, we want a dynamic mechanism that can enforce write-allocate when writes have reuse, and enforce \hl{mostly} write-no-allocate \hl{(RRIP)} when writes have no reuse, to optimize for both cache space and write traffic. Such a dynamic mechanism needs methods to: (a) observe reuse of write-allocated lines, (b) learn reuse characteristics of write-allocated lines, and (c) enforce appropriate write-allocate or write-no-allocate policy. To this end, we propose {\em Dynamic Write-allocate Policy (DWP)}.

\subsection{Dynamic Write-Allocate Policy} 


Figure~\ref{fig:dynamic_writeback} shows the structures we need to implement our Dynamic Write-allocate Policy. We need structures to implement: (a) observing reuse for write-allocated lines, and (b) learning the reuse, so that we can make informed decisions. (a) To observe write-allocate reuse, we need a bit to mark lines that were installed via write-allocate (\textit{WA bit}), and a bit (\textit{R bit}) to remember if this line was reused in its lifetime. WA-bit is set on install-time (if it is a write-allocated line), and R-bit is set on read or write to the line. On eviction, these bits inform us if a write-allocated line was reused or not. And (b) we need a structure to learn the reuse of write-allocated lines. We implement the learning structure with a small saturating counter. This saturating counter is incremented on observing reuse (R=1) of write-allocated lines, and decremented on observing no-reuse (R=0) of write-allocated lines. The combination of (a) and (b) enable us to determine if write-allocated lines have reuse or not. Finally, we add thread-id to both the observation and learning phase to make the policy thread-aware. This enables us to determine which threads are likely to reuse write-allocated lines and make per-thread policy decision.


\begin{figure}[htb] 
	\vspace{-0.10in}
	\centering
	\includegraphics[width=1.0\columnwidth]{FIGURES/dynamic_writeback.pdf}
	\vspace{-0.15in}
	\caption{Dynamic Write-allocate Policy \textit{observes} reuse of writes, \textit{learns} in per-core usefulness counters, and \textit{enforces} write-allocate / write-no-allocate.}
	\label{fig:dynamic_writeback} 
	%\vspace{-0.10in}
\end{figure}

Observation and Learning phase enables us to determine the likelihood of each thread to reuse its write-allocated lines. In Figure~\ref{fig:dynamic_writeback}(c), a non-zero counter indicates a thread is likely to reuse write-allocated lines, and a zero counter indicates a thread is unlikely to reuse write-allocated lines. If the counter is non-zero, we enforce a write-allocate policy \hl{by overriding the RRIP decision (install line and update RBT)}. This enables us to use the DRAM-cache as a write buffer and reduce writes to non-volatile memory. And, if the counter is zero, we default to RRIP, which allows us to \hl{mostly} write-no-allocate. This enables us to use the cache more effectively by preserving resident lines. DWP enables a cache to enact appropriate write-allocate decision at run-time.  DWP requires storage of 24 bits.


\subsection{Impact of DWP on Write Traffic} 

Figure~\ref{fig:dynamic_writeback_traffic} shows the L4 writeback traffic for Always-Install, and three flavors of ETR: write-unaware, allocate-on-write-miss, and DWP.   ETR with allocate-on-write-miss reduces write traffic for write-allocate-friendly workloads such as \textit{bc twi}, to achieve 33\% reduction in L4 writebacks compared to the baseline always-install policy. Our proposed DWP is effective at dynamically choosing write-allocate as it achieves write traffic reduction similar to allocate-on-write-miss. 

%But, write-allocate can hurt capacity-sensitive workloads such as \textit{pr web} or \textit{zeusmp}.

%DWP reduces 33\% of write traffic.


\begin{figure}[htb] 
	\vspace{-0.0 in}
	\centering
  \hspace*{-.45cm}\includegraphics[width=1.09\columnwidth]{GRAPHS/mpki_w.pdf}
	\vspace{-0.20in}
	\caption{Write traffic for Baseline (Always Install), ETR (Write Unaware), ETR (Allocate on Write-Miss), and ETR (Dynamic Allocate) in terms of L4 writebacks per 1000 instructions (WBPKI).    DWP reduces WBPKI by 33\%.}
	\label{fig:dynamic_writeback_traffic} 
	\vspace{-0.05in}
\end{figure}


\subsection{Impact of DWP on Performance} 


Figure~\ref{fig:shipwb_perf} shows the performance of three flavors of ETR: write-agnostic, allocate-on-write-miss, and DWP. We also show State-in-SRAM with the DWP policy as it can also benefit from DWP. ETR with allocate-on-write-miss  benefits write-allocate-friendly workloads such as \textit{bc twi}, \textit{milc}, and \textit{mixes}. But, write-allocate can hurt capacity-sensitive workloads such as \textit{pr web} or \textit{zeusmp}. Meanwhile, ETR with DWP is able to dynamically decide between write-allocate and ETR (mostly write-no-allocate) to outperform either policies to reach 19.4\% speedup, with no workloads experiencing slowdown. 

%DWP incurs negligible storage overhead (24 bits more than ETR).



%%%% GRAVEYARD %%%%%%%%%%

\ignore{
\section{Design: QoS-Aware Replacement}

QoS. 
But, workloads participating in sharing can get their space consumed by higher mpki workloads. Can we ensure performance? Define QoS as perf relative to partitioned is above a threshold.

Determine when workloads breaking qos
Get partitioned perf: Sample 1% sets, and run srrip on individual partitions using extra space (just tags) in ecc to estimate hitrate_srrip_partition. Works because storage is cheap, but bw is expensive.
Get shared perf: get hit-rate per thread. Tid stored.
If hit-rate diff >5%, protect workload (Taker). Otherwise, giver (does sharing, but yields to taker)
Enforce
If same, do default.
If taker resident and giver incoming, bypass.
If giver resident and taker incoming, always-install.

}

%Fortunately, we find that the SHiP observing and learning mechanism is a good fit. On write-install, we simply write the signature as core\_id (as there is no valid PC information on writebacks). If we follow the same observing and learning process, we will be able to learn if written lines are re-used or not. If there is reuse (SHCTR[core\_id]\textgreater0), we implement Always-Install for writes to emulate a write-back cache. If there is no reuse (SHCTR[core\_id]==0), we default to normal RRIP install policy. This allows us to appropriately reduce main-memory write traffic when writes are reused, and improve cache utilization when writes are unlikely to be reused.

%Figure~\ref{fig:shipwb_perf} shows the performance of BASE-SHiP, write-aware SHiP (DRAM-SHiP), and the impractical state-in-SRAM SHiP (SRAM-SHiP). Write-aware SHiP further improves the performance of SHiP for write-back-friendly workloads of \textit{bc twi}, \textit{milc}, and \textit{mixes}. Write-aware SHiP achieves an overall 21\% speedup with no workloads experiencing slowdown and with negligible storage overhead (\textless 2KB).

%This is because certain workloads have write traffic and can re-use the data.


%Figure~\ref{fig:dynamic_writeback} shows the writeback miss per thousand instructions for Always-Install and ETR. Of notice, ETR has increased write traffic for \textit{bc twi} compared to Always-Install. This is because Always-Install inherently implements Write-Allocate on write miss. Figure~\ref{fig:writeback}(b) shows that a write-allocate policy can mitigate memory writes when writes have reuse. Meanwhile, ETR treats read-miss and write-miss identically and often bypasses for write-misses, effectively implementing Write-No-Allocate. Figure~\ref{fig:writeback}(a) shows that ETR's mostly write-no-allocate policy avoids allocating cache space for write-misses, which can save space when writes have no reuse. However, such a write-no-allocate policy 

%We have previously treated write-misses with the same install policy as read-misses. However, in the case of a write-miss, bypassing the cache would mean directly writing to our write-sensitive non-volatile main-memory, shown in Figure~\ref{fig:writeback}(a). This effectively means our RRIP policy is often implementing write-no-allocate (or write-around). In the case that writes are not reused, a write-around policy optimizes for cache space by writing directly to memory, with no adverse effects. However, some workloads do see reuse for written lines, and, a write-back policy would be able to reduce the number of writes to memory, shown in Figure~\ref{fig:writeback}(b). We need a mechanism to determine dynamically when it is appropriate to write-around or write-back.


%We observe that write-allocate policy has significant impact on performance. A major reason for this impact is because we assume a write-sensitive non-volatile memory. If a policy increases write traffic, the increased writes can delay the completion of reads and cause longer read latency.

%If a policy improves hit-rate but increases write traffic, the increased writes can delay the completion of reads and cause longer read latency. As ETR treats read-misses and write-misses identically, ETR

%A good replacement policy for an NVM-backed system should be able aware of additional write traffic caused. 
%So, why does our ETR policy cause increased writes for \textit{bc twi}?
%So why does write policy have so much impact on performance.



%On line install, we set the WA bit if the line was installed under write-allocate. 

%To determine when it is appropriate to write-back or write-around, we need a mechanism that can observe re-use for written lines. Figure~\ref{fig:dynamic_writeback} shows our thread-aware dynamic writeback mechanism. To \textit{observe}, on install, we simply to maintain 1-bit to store whether or not the line is a write (is\_store), \texttildelow3-bit for thread awareness (core\_id), and 1-bit if the line is reused or not (has\_reuse). On read or write to a stored line, we update the has\_reuse bit (note: we sample 1\% sets to reduce this update traffic). On eviction, we can know if a particular thread reused a written line. Based on this observed reuse of writes, we can \textit{learn} and increment or decrement a per-core counter accordingly to know how likely a particular core is to reuse its written lines. If stores have reuse, we should always-install writes with write-back policy to avoid increasing main memory write traffic. If stores have no reuse, we default to RRIP and mostly-bypass to improve cache usage.

% for \textit{bc twi}, in Figure~\ref{fig:dynamic_writeback}



